10Cache: Heterogeneous Resource-Aware Tensor Caching and Migration for LLM Training

Training large language models (LLMs) in the cloud faces growing memory bottlenecks due to the limited capacity and high cost of GPUs. While GPU memory offloading to CPU and NVMe has made large-scale training more feasible, existing approaches suffer from high tensor migration latency and suboptimal device memory utilization, ultimately increasing training time and cloud costs. To address these challenges, we present 10Cache, a resource-aware tensor caching and migration system that accelerates LLM training by intelligently coordinating memory usage across GPU, CPU, and NVMe tiers. 10Cache profiles tensor execution order to construct prefetch policies, allocates memory buffers in pinned memory based on tensor size distributions, and reuses memory buffers to minimize allocation overhead. Designed for cloud-scale deployments, 10Cache improves memory efficiency and reduces reliance on high-end GPUs. Across diverse LLM workloads, it achieves up to 2x speedup in training time, improves GPU cache hit rate by up to 86.6x, and increases CPU/GPU memory utilization by up to 2.15x and 1.33x, respectively, compared to state-of-the-art offloading methods. These results demonstrate that 10Cache is a practical and scalable solution for optimizing LLM training throughput and resource efficiency in cloud environments.

==> included/5-implementation_detail.tex <==
\section{Implementation Details}
\label{implementation_detail}

% \arb{perhaps we can make this a subsection of evalution, as this is just a brief system... there we can start with:

% We have implemented \proj....
% }

\proj~is built on top of DeepSpeed~\cite{deepspeed}, an open-source framework highly optimized for LLM training and developed on PyTorch~\cite{pytorch}. We enhance DeepSpeed ZeRO-Infinity~\cite{zero_infinity-SC21} by implementing more efficient placement strategies for model parameters and optimizer states across heterogeneous memory. Additionally, we introduce intelligent scheduling policies for tensor migration and advanced memory management to improve training throughput. Since \proj~seamlessly integrates with DeepSpeed, any LLM training workflow compatible with DeepSpeed can run on \proj~without modification, enhancing both the practicality and efficiency of the system. For GPU memory profiling, \proj~leverages the nvidia-smi tool to monitor used and available GPU memory. To track CPU memory usage, it employs Psutil, a cross-platform Python library.

% \proj is implemented on top of DeepSpeed \cite{deepspeed}. DeepSpeed is an open-source framework highly optimized for LLM training built on top of PyTorch \cite{pytorch}. We implement more efficient model paramaters, optimizer states placement on heterogeneous memory, smart scheduling policies for tensor migration along with memory management on top of DeepSpeed ZeRO-Infinity \cite{zero_infinity-SC21} feature to get better training throughput. As \proj is built on top of DeepSpeed, any LLM training with DeepSpeed framework is also possible with this system without any modification. It makes our system more practical and powerful. For GPU memory profiling, \proj utilizes nvidia-smi tool to monitor both used and free GPU memory. Again, for available and used CPU memory, \proj uses Psutil, a Python cross-platform library.

% \REV{While section 3 (\proj Design) is fairly comprehensive, section 4 (Implementation Details) feels a little bit light. In particular, more details about GPU memory profiling would be valuable. nvidia-smi is mentioned as being employed, but I think some justification is merited as to why nvidia-smi is sufficient for this use-case. For example, if PyTorch reserves more memory than it is actively using, it is my understanding that nvidia-smi will report all of the reserved memory as being "used." Are limitations of nvidia-smi not relevant to this work?}

